Hybrid tracker based optimal path tracking system for complex road environments for autonomous driving

Path tracking system plays a key technology in autonomous driving. The system should be driven accurately along the lane and be careful not to cause any inconvenience to passengers. To address such tasks, this paper proposes hybrid tracker based optimal path tracking system. By applying a deep learning based lane detection algorithm and a designated fast lane fitting algorithm, this paper developed a lane processing algorithm that shows a match rate with actual lanes with minimal computational cost. In addition, three modified path tracking algorithms were designed using the GPS based path or the vision based path. In the driving system, a match rate for the correct ideal path does not necessarily represent driving stability. This paper proposes hybrid tracker based optimal path tracking system by applying the concept of an observer that selects the optimal tracker appropriately in complex road environments. The driving stability has been studied in complex road environments such as straight road with multiple 3-way junctions, roundabouts, intersections, and tunnels. Consequently, the proposed system experimentally showed the high performance with consistent driving comfort by maintaining the vehicle within the lanes accurately even in the presence of high complexity of road conditions. Code will be available in https://github.com/DGIST-ARTIV.

==> F_acknowledgement/acknowledgement.tex <==
%This Research is supported by DGIST Undergraduate Group Research Program (UGRP).
%본 연구는 과학기술정보통신부에서 지원하는 DGIST 기관고유사업에 의해 수행되었습니다(21-BRP-09 \& 21-BRP-08).
This research was conducted by the DGIST institution-specific project supported by the Ministry of Science and ICT (21-BRP-09 \& 21-BRP-08).

==> MainDocs/background/a_Path_tracking_algorithm.tex <==
\subsection{Path Tracking Algorithm}
Generating a path that the vehicle should take to its destination and following the generated path are the most essential parts of an autonomous vehicle.

There are three types of path tracking algorithms, which are divided into geometric model-based, kinematic model-based, and dynamic model-based algorithm \cite{snider2009automatic}. Among these three path tracking algorithms, the simplest algorithm type is the geometric model-based path tracking algorithm such as Pure pursuit, Stanley controller, and Vector pursuit. % \textcolor {blue} {The most commonly used algorithms are  \cite{patnaik2020design}.}
 
The algorithms used in this paper are Pure pursuit and Stanley controller. Pure pursuit and Stanley controller use the same bicycle model regardless of vehicle type, so that the calculation is simple and easy to apply compared to other path tracking algorithms \cite{cibooglu2017hybrid}. Unfortunately, it was reported that these two algorithms work well only on low-speed and general roads \cite{kim2020comparative}. Conversely, when the curvature of the road turns to large or the speed of the vehicle becomes high, it is unable to follow the generated path. Therefore, if kinematic model and dynamic model are used, tracking performance can be improved in more diverse environments. However, the above simple algorithms(Pure pursuit and Stanley controller) were appropriately modified and used to achieve maximum efficiency with limited computer performance.
 
Pure pursuit's tracking performance depends on the look-ahead distance, which leads importantly to set an appropriate look-ahead distance. Otherwise, unlike other path tracking algorithms, Stanley controller does not use a look-ahead distance, so parameters have not to be tuned \cite{amer2018adaptive}. Comparing multiple path tracking algorithms \cite{snider2009automatic},  Pure pursuit shows robust to low-speeds and large errors, but it does not work well at high-speeds \cite{park2014development, dominguez2016comparison}.
However, Stanley controller has a faster rate of convergence to the ideal path than the Pure pursuit, but there are cases where the steering angle sometimes diverges on a road with a large curvature.
 
%\textbf{여기 수정 In order to apply these two algorithms in various situations}, 
This paper modified the existing algorithms to minimize the disadvantages mentioned above and apply in various situations.

% 저자 없애기 전 버전
\begin{comment}
Generating a path that the vehicle should take to its destination and properly following the generated path are the most essential parts of an autonomous vehicle.

According to path tracking algorithm classification of Snider et al. \cite{snider2009automatic}, there are three types of path tracking algorithms and the types are divided into geometric model-based, kinematic model-based, and dynamic model-based algorithm. Among these three path tracking algorithms, the simplest algorithm type is the geometric model-based path tracking algorithm.In accordance with path tracking algorithm review of Patnaik et al.  \cite{patnaik2020design}, the most commonly used algorithms are Pure pursuit, Stanley controller, and Vector pursuit.
 
The algorithms used in this paper are Pure pursuit and Stanley controller. According to research of Cibooglu et al.  \cite{cibooglu2017hybrid}, Pure pursuit and Stanley controller %do not use dynamic models, but 
use the same bicycle model regardless of vehicle type, so that the calculation is simple and easy to apply compared to other path tracking algorithms. According to Kim's analysis of these two algorithms \cite{kim2020comparative}, these algorithms work well only on low-speed and general roads. On the other hand, when the curvature of the road \textcolor{red}{turns to} large or the speed of the vehicle \textcolor{red}{becomes} high, % there is a disadvantage that 
it is unable to follow the generated path. Therefore, if kinematic model and dynamic model are used, tracking performance can be improved in more diverse environments. However, the above simple algorithms(Pure pursuit, Stanley controller) were appropriately modified and used to achieve maximum efficiency with limited computer performance.
 
Pure pursuit's tracking performance depends on the look-ahead distance, \textcolor{red}{which leads importantly} to set an appropriate look-ahead distance. Otherwise, unlike other path tracking algorithms, Stanley controller does not use a look-ahead distance, so \textcolor{red}{parameters have not to be tuned} \cite{amer2018adaptive}. According to Snider's \cite{snider2009automatic} comparing multiple path tracking algorithms, Park's \cite{park2014development}, and Dominguez's \cite{dominguez2016comparison}, Pure pursuit is robust to low-speeds and large errors, but it does not work well at high-speeds. However, Stanley controller has a faster rate of convergence to the ideal path than the Pure pursuit, but there are cases where the steering angle \textcolor{red}{sometimes} diverges on a road with a large curvature.
 
\textcolor{red}{This paper modified the existing algorithms to minimize the disadvantages mentioned above and apply in various situations.}
\end{comment}

%, which will be described in section \ref{subsection: path tracking algorithm}.

\begin{comment}
In order to apply these two algorithms in various situations, it was modified to minimize the disadvantages of the existing algorithm.

These two algorithms were modified 

이 두 가지 알고리즘을 다양한 상황에서 모두 적용시키기 위하여 기존의 알고리즘의 단점을 최소화하도록 변형하였다.

이 두 가지 알고리즘은 단점을 최소화하도록 변형되었고 다양한 상황에서 모두 적용되었다.

In this paper, these two algorithms were modified to minimize their disadvantages and applied in various situations.
\end{comment}


==> MainDocs/background/b_Lane_detection_networks.tex <==
\begin{comment}
딥러닝 이미지 프로세싱에 대한 많은 Related work, 동향
Ensemble, Boost --> Processing
한정된 시간 높은 결과를 얻기위해서 주변 논문들은 어케 했냐
\end{comment}

\subsection{Lane Detection Networks}

Studies about end-to-end network performance for lane detection are as follows. PointLaneNet \cite{chen2019pointlanenet} redefined the lane structure and lane distance to facilitate the training of the network. PINet \cite{ko2020key} combined point estimation and point instance segmentation, but there were limitations in the presence of the local occlusions or unclear lanes. Lightweight model ENet-SAD applied SAD to ENet\cite{paszke2016enet} has emerged. Hou et al. proposed lightweight model ENet-SAD with Self Attention Distillation(SAD) to existing ENet \cite{paszke2016enet}. SCNN \cite{pan2018SCNN} and ENet-SAD obtain diverse and rich contextual information to solve these limitations.
In the autonomous driving system, various methods are attempted to reduce the delay from sensor recognition to vehicle maneuvering as much as possible. In particular, deep learning is now considered essential in the perception field, but it has disadvantages that it cannot secure both processing speed(inference time) and performance(accuracy) due to the limitation of GPU hardware. However, processing performance varies depending on the size of the network parameter or the computational complexity of the layer. The recent deep learning methodologies have proposed various methods to solve these obstacles. ENet-SAD improved the processing speed by applying self-attention approach. Its processing speed  secured 10 times faster comparing with SCNN. In addition, a method of actively using conventional computer graphics technology has been proposed to improve the performance of deep learning algorithms. This paper proposed fast and accurate lane processing algorithm using the results of ENet-SAD. A low-latency and highly reliable lane detection system has been designed.

% 우리 연구팀은 이러한 상황 속에서 ENet-SAD 같은 차선 세그먼테이션 딥러닝 네트워크 전용으로 빠르게 차선 데이터를 정합하여 Points 또는 데이터 처리가 용이하도록 하는 고속 차선 정합 시스템에 초점을 두었다.

 \begin{comment}
  낮은 전력을 소모해야하는 모바일 디바이스에서 real time segmentation을 하기 위해서는 빠른 처리 속도와 높은 정확도로 최적화된 신경망이 필요하다. 선행 연구는 Lane detection을 위한 end-to-end networks를 제안했다. \cite{chen2019pointlanenet}에서,  chen은 네트워크의 학습을 용이하게 하기위해서 차선구조와 차선 거리를 재정의한 PointLaneNet을 제안했다. \cite{ko2020key}에서, Ko는 point estimation과 point instance segmentation을 결합한 PINet을 제안했으나 local occlusions나 unclear lanes가 있을 경우 한계가 있다고 주장했다. hou는 기존에 있던 Paszke의 ENet\cite{paszke2016enet}에 self-attention approach를 적용한 lightweight의 model ENet-SAD를 제안하였고,  ENet-SAD는 더욱 다양하고 풍부한 contextual information을 얻어 Pan의 SCNN \cite{pan2018SCNN}보다 10배 빠른 13.4ms의 성능을 보인다고 주장했다.\cite{hou2019learning} 
  우리는 hou의 ENet-SAD를 사용하였고, 이 네트워크의 성능을 data preparation을 통하여 향상시켰다. % (이 부분 제거) lane segmentation을 후처리하고 lane fitting하여 차선 종속 주행의 주행유도선을 제공하고자 했다.

 
 In order to perform real time segmentation in a mobile device that consumes low power inevitably, a neural network optimized with high processing speed and high accuracy is required. Previous studies have proposed end-to-end networks for lane detection. Chen proposed PointLaneNet \cite{chen2019pointlanenet}, which redefined the \textbf{lane structure and lane distance 원본에서 쓰는 개념 가져오기} to facilitate the training of the network. Ko proposed a PINet \cite{ko2020key} that combines point estimation and point instance segmentation, but there are limitations in the presence of the local occlusions or unclear lanes. \textcolor{blue}{here 위에서 똑같은 말 반복} Hou proposed lightweight model ENet-SAD with self-attention approach to existing Paszke's ENet \cite{paszke2016enet}. Hou argued that ENet-SAD achieves 13.4ms, 10 times faster than Pan's SCNN\cite{pan2018SCNN}, by obtaining diverse and rich contextual information. We used ENet-SAD by Hou and improved the performance of this network through data preparation.
 \end{comment}
 
\begin{comment}
 ENet은 낮은 latency 연산으로 구성된 새로운 딥 뉴럴 네트워크 구조이다. ENet은 Encoder와 Decoder로 이루어져 있다. Encoder 부분은 5개의 병목 블록 3개로 이루어져 있으며 마지막 블록에서는 다운 샘플링하지 않는 구조이다. Decoder 부분은 max pooling이 max unpooling으로 대체되고, padding은 bias가 없는 spatial convolution으로 대체되었다. ENet의 최종 architecture의 모양을 결정하는데, feature map resolution, early downsampling, decoder size, nonlinear operations, information-preserving dimensionality changes, factorizing filters, dilated convolutions, regularization을 고려하였다. 그 결과, 해상도 640*360 입력일 때 10fps 성능을 보였다. SegNet대비 18배 이상 빠르고 75배보다 적은 FLOPS, 79배 적은 파라미터 값을 가지며 더 나은 정확도를 보였다.
 
ENet은 segmentation maps에 강하게 의존하는데, lane이 길고 얇을 경우 lane이 없다고 인식한다. lane annotation 자체의 width를 늘리는 방식도 그럴듯 해 보이지만 performance가 낮다. ENet-SAD의 구조는 ENet 딥러닝 네트워크에 작은 network와 AT-GEN을 추가한 형태이다. 전 layer를 모방하여 다음 layer를 만들어낸다. 자기 스스로에게서 파생된 attention maps를 만들어 학습하는 것으로 inference time에 영향을 주지 않고 길고 얇은 lane에 대한 문제를 해결한다. ENet-SAD는 우리가 전처리로 해줄 초반 labeling을 제외하고 부가적인 labeling이나 외부의 supervision이 필요하지 않으며, 비교적 가벼운 차선 인식 딥러닝 네트워크이다. ENet에 SAD를 추가한 결과 lower level의 layer들의 contextual information을 더욱 다양하고 풍부하게 재정의했고 붐비는 도로, 적은 양의 빛이 있는 상황에서도 detection performance가 떨어지지 않을 뿐만 아니라 visual attention도 향상 시켰다. 특히, open datset 중 CULane으로 학습시키고, test했을 경우 runtime이 13.4ms로 약 74fps의 성능을 낸다.
\end{comment}

==> MainDocs/background/c_Ensemble_method.tex <==
\subsection{Ensemble method}
\begin{comment}
raw image에서 차선을 인식하고 차선 segmentation image에서 차선에 대한 정보를 뽑아내는 것은 주행유도선을 제공하는 데 꼭 필요한 과정이다. 머신러닝에서는 단일 모델만을 이용하여 성능을 끌어올리는 데에는 한계가 있기 때문에 여러 모델의 예측을 결합하여 최종 결과가 더 나은 성능을 내도록하는 방법인 ensemble method를 사용하고 있다. ensemble method에는 voting, Bagging 등 다양한 방법이 존재한다. voting은 동일한 dataset에 대하여 다양한 알고리즘이 예측한 결과에 대하여 투표하여 최종 결과를 선택한다. voting에는 hard voting과 soft voting이 있다. hard voting은 여러 모델에서 예측한 결과 중 단순히 가장 많은 표를 얻은 결과를 선택하는 것이다. soft voting은 여러 모델에서 예측한 결과의 probability를 합해 가장 높은 결과를 선택하는 것이다. Bagging은 중첩을 허용하여 서로 다르게 샘플링한 데이터셋에 대하여 하나의 알고리즘이 예측한 결과들을 투표로 최종 결과를 결정하는 방식이다. 본 연구팀은 빠른 차선 정합 알고리즘에서 빠른 연산속도를 위하여 병렬적으로 처리가 가능한 soft voting의 방식을 채택하였다. \cite{teow2002robust}의 Teow는 soft voting을 채택하여 손글씨 인식에서 가장 좋은 결과를 얻을 수 있었고,  \cite{li2017bearing}의 Li는 soft voting을 이용하여 신호 세그먼트의 예측 결과 집계의 정확도와 안정성을 높였다.

Zhou는 \cite{zhou2005training}에서 cost-sensitive neural networs를 훈련하는데 soft voting 방식

\textbf{soft voting을 이용한 예시들을 나열, 딥러닝, 리니어 리그레션의 성능을 높인 것을 찾던가 등등, Ref 채우기}
같은 segmentation image의 차선들에 대한 fitting 식을 결정 할 때, 차선에 대한 식의 분산을 metric으로 하여 가장 낮은 분산을 가진 결과를 최종 결정하였다.
\end{comment}
Recognizing lanes in raw images and extracting information about lanes in segmentation images are necessary processes. In machine learning, ensemble method combines predictions from multiple models rather than a single model, so that the final result achieves better performance. The types of ensemble methods are Voting and Bootstrap Aggregating(Bagging). %\textcolor{red}{The former method}
The Voting method compares the results predicted by various algorithms for the same dataset and chooses the final result. There are types of voting: soft voting and hard voting. Hard voting simply chooses the results that received the most votes among the predictions from different models. Soft voting selects the highest result by summing the probability of the predicted results from different models. Bagging is a method of voting to determine the final results predicted by one algorithm on various datasets sampled differently by allowing overlap. In Teow's handwriting recognition research, the best results came out by adopting soft voting \cite{teow2002robust}. Soft voting increased the accuracy and stability of aggregation as a result of prediction in signal segments \cite{li2017bearing}. This paper adopted soft voting that can be parallel processing guaranteed fast computational speed in lane fitting algorithm.

==> MainDocs/introduction.tex <==
\PARstart{I}{n} recent years, the requirements for the driving system of the autonomous vehicle are increasing in difficulty according to levels of driving automation proposed by SAE \cite{sae2014taxonomy}. In Level 4 (or above) of vehicle autonomy, the vehicle should perform the main driving and request humans to transfer control only in special circumstances or in areas where autonomous driving is not possible. For this reason, combining the two fields of perception and control algorithm is emerging as a very important area in autonomous driving. Hence, end-to-end deep learning tracking algorithms \cite{tran2019robust, neven2018towards, xing2018advances} or methods using reinforcement learning \cite{khan2019latent} have been studied, but these methods are difficult to response flexible changes in the surrounding environment.

% In order to take full advantage of deep learning,
The deep learning based lane detection and the GPS based driving path tracking were also applied to deal with complex road environments. The control method used geometric model-based path tracker, Pure pursuit and Stanley controller, which are widely used in the control field.This research proposes a lane tracking system that can pass through not only highways and motorway roads, but also urban and complex road environments.
In high-speed and low-speed, tunnel, and steep curve, the system quickly changed the appropriate tracking method and reflected it in driving stability for different speeds. In lane detection, the algorithm designed to process the deep learning method has been applied the three lane fitting methods in parallel to provide the most optimized path.

The modified path tracking algorithm is designed to simultaneously process vision data to GPS data, in other words, local and global coordinates. Vision and GPS based driving guidance lines cause uncomfortable driving textures when driving along the lines. Accurately following the lane is also an act that does not take into account driving stability or driver acceptance. To solve this problem, we suggested an optimal path tracking algorithm to ensure high driving stability and comfortableness have been studied in this paper.

This optimal path tracking algorithm appropriately selects the most stable tracker out of modified trackers, so called Hybrid tracker based optimal path tracking system. This system receives sensor information at the same time as each tracker calculation, estimates the driving environment, and transfers the control authority to the most suitable tracker. Due to the difference in the computational speed of each path tracking algorithm, the driving stability of the vehicle can be changed.

Therefore, we configured the parallel system to minimize the stability degradation. This method guarantees consistent driving stability even in various driving environments with different characteristics. Furthermore, it has the advantage that additional correction of the computational speed is not required on the hybrid system even if each tracker is modified. Finally, this paper proposes the hybrid tracker based optimal tracking system capable of driving in a complex road environment, and the result of applying the proposed system in various environments guarantees a high degree of driving stability and accuracy.

The development of seamless proposed system in complex road environment on various speed is essential as the current trend of increasing the driving authority of the vehicle itself. We installed the system in a vehicle and confirmed its performance at the DGIST campus and high-speed driving proving ground. To sum up, the contribution points of this paper are as follows; deep learning based lane detection and fast optimal lane processing algorithm; and the hybrid tracker based optimal path tracking system that ensures high driving stability.

